Universally Sloppy Parameter Sensitivities in Systems Biology

Quantitative computational models play an increasingly important role in modern biology. Such models typically involve many free parameters, and assigning their values is often a substantial obstacle to model development. Directly measuring \emph{in vivo} biochemical parameters is difficult, and collectively fitting them to other data often yields large parameter uncertainties. Nevertheless, in earlier work we showed in a growth-factor-signaling model that collective fitting could yield well-constrained predictions, even when it left individual parameters very poorly constrained. We also showed that the model had a `sloppy' spectrum of parameter sensitivities, with eigenvalues roughly evenly distributed over many decades. Here we use a collection of models from the literature to test whether such sloppy spectra are common in systems biology. Strikingly, we find that every model we examine has a sloppy spectrum of sensitivities. We also test several consequences of this sloppiness for building predictive models. In particular, sloppiness suggests that collective fits to even large amounts of ideal time-series data will often leave many parameters poorly constrained. Tests over our model collection are consistent with this suggestion. This difficulty with collective fits may seem to argue for direct parameter measurements, but sloppiness also implies that such measurements must be formidably precise and complete to usefully constrain many model predictions. We confirm this implication in our signaling model. Our results suggest that sloppy sensitivity spectra are universal in systems biology models. The prevalence of sloppiness highlights the power of collective fits and suggests that modelers should focus on predictions rather than on parameters.

==> Dataset1/README <==
Each directory corresponds to a model. 

hessian.dat is the the \Chi^2-hessian. hessian_keys.dat lists the parameters in the order they enter the hessian.

The .py files in the directories are:
Nets.py: Creates the Networks (conditions) that we'll consider for the model.
reproduction.py: When run, produces graphs for the various conditions that can
                 be compared with the original publication to help confirm that
                 we've successfully implemented their model.

To generate the \Chi^2-Hessians for a specific model, use
python runModels.py <model directory name>

When finished, the model directory will contain a number of hess_dict.*.bp files, one for each condition. These correspond to the individual terms in the sum for H^{\chi^2}. It will also regenerate hessian.dat and hessian_keys.dat.

Fig1B_spectra_plot.py, Fig1C_alignment_plot.py and Fig3_plot.py create Figures 1B,C and 3, respectively.

Brown_2004/prediction.py recreates Figure 4B and those in Text S2.

S4_rescaled_Brown_plot.py and S5_plot.py recreate the figures in Text S4 and S5.

The scripts were all run with SloppyCell version 0.81. Updated versions to adjust to changes in SloppyCell are available from the authors.

